Debiased Distillation by Transplanting the Last Layer

Deep models are susceptible to learning spurious correlations, even during the post-processing. We take a closer look at the knowledge distillation -- a popular post-processing technique for model compression -- and find that distilling with biased training data gives rise to a biased student, even when the teacher is debiased. To address this issue, we propose a simple knowledge distillation algorithm, coined DeTT (Debiasing by Teacher Transplanting). Inspired by a recent observation that the last neural net layer plays an overwhelmingly important role in debiasing, DeTT directly transplants the teacher's last layer to the student. Remaining layers are distilled by matching the feature map outputs of the student and the teacher, where the samples are reweighted to mitigate the dataset bias. Importantly, DeTT does not rely on the availability of extensive annotations on the bias-related attribute, which is typically not available during the post-processing phase. Throughout our experiments, DeTT successfully debiases the student model, consistently outperforming the baselines in terms of the worst-group accuracy.

==> contents/method_edit2.tex <==
\section{Method: Debiased Teacher Transplant (DeTT)}

Our method distills teacher's feature map and reuses classifier not to train bias-sensitive module, classifier layer. 
With this method, we can distill and reuse teacher's knowledge with less bias without group annotation.
Also, characteristic of feature distillation with biased dataset is analyzed through different hyperparameter setting and ablation studies.
Leftover bias in feature map is removed by weak sample upweighting.

\subsection{Feature distillation and Reusing teacher module}
\label{subsec:simkd}
Vanilla knowledge distillation \cite{hinton2015distilling} uses teacher model output $p_T = g_T(\phi_T (x))$ as knowledge to be distilled.
Its distillation loss function to be minimized is represented as follows:
\begin{equation}
    \mathcal{L}_{\mathrm{KD}}=(1-\alpha)\mathcal{L}_{\mathrm{CE}}(y, p_S) + \alpha \mathcal{L}_{\mathrm{KL}}(p_T, p_S)
    \label{eq:distill}
\end{equation}
$\mathcal{L}_{\mathrm{CE}}$ and $\mathcal{L}_{\mathrm{KL}}$ are cross-entropy loss and Kullback–Leibler divergence (KLDiv) loss respectively.
$\alpha$ is a hyperparameter for distillation ratio. 

%\input{resource/fig/method}

%Above part is preliminaty part
Previous research \cite{izmailov2022feature} shows that classifier layer is more sensitive to bias in dataset and debiasing algorithm compared with feature map.
We do not want to take risk of being biased by training classifier.
From this motivation, our method reuse $g_T(\cdot)$ with projector $P(\cdot)$ to fit dimension (or no projector if dimension already fits)  and only use optimization function for feature map as follows \cite{chen2022knowledge}:
\begin{equation}
    \mathcal{L}_{\mathrm{KD}}=\mathcal{L}_{mse}(\phi_T (x), P(\phi_S (x)))
\end{equation}
We use mean square error as loss ($\mathcal{L}_{mse}$) for simplicity.
However, we show it is not fully debiased for some imbalanced dataset in \ref{sec:AblaUpweight}.
We think that frequency of feature activation appearance is different and it works as bias in feature map.

\subsection{Upweight samples without group annotation}
\label{subsec:upweight}
To solve problem mentioned above subsection, our method needs to upweight data sample to remove leftover bias. 
Samples to be upweighted is selected by \textit{identification model} trained via empirical risk minimization(ERM) whose architecture is identical with that of student network \cite{liu2021just}.
Training example which failed to be optimized in identification model (i.e. expected to be minor group sample).
Dataset used for knowledge distillation is upweighted dataset $\mathcal{D}_{kd}$ constructed by concatenating original dataset $\mathcal{D}$ and upweighted samples $\mathcal{D}_{\lambda_{up}}$ when $\lambda$ is upweight hyperparameter.
In our work, those weak debias technique is sufficient for removing bias in feature map level.


==> contents/my_memo.tex <==
*** potential reference ***


\cite{stanton2021does} : knowledge distillation performance gain is due to label smoothing effect -> regularization -> performance up\\
knowledge distillation itself can help debiasing.



*** Things to do ***
naive kd 와 vanilla kd 통일


distill 상황에서 bias가 mainly distill되는 문제가 있음.

Motivation

DeTT 설명

JTT{
baseline dataset 설명, 절대성능 (erm과 비교)

analyze method

다른 robust training과 비교
}

*appendix 
dataset specific
t-sne




=================================Warehouse
In summary, we suggest well-performing baseline for robust knowledge distillation and analyze what knowledge is distilled through feature map calculated with spurious correlated data.

==> resource/fig/tsne_celeb/celeb_tsne.tex <==
\begin{figure*}[t]
  \centering
%    \begin{center}
    %\framebox[4.0in]{$\;$}
    \subfigure[Feature map from first block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_celeb/layer1_celeb.pdf}
      \label{fig:celebsub1}
    }
    \subfigure[Feature map from third block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_celeb/layer3_celeb.pdf}
    %  \subcaption{A subfigure}
      \label{fig:celebsub3}
    }
        \subfigure[Feature map from fourth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_celeb/layer4_celeb.pdf}
    %  \subcaption{A subfigure}
      \label{fig:celebsub4}
    }    
        \subfigure[Feature map distilled in DeTT]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_celeb/layer6_celeb.pdf}
    %  \subcaption{A subfigure}
      \label{fig:celebsub6}
    }    
    
    \caption{
    In lower feature map, data classification is dominant to background feature (orange-green pair and red-blue pair).
    It means that it is not necessary to distill lower level feature map.
    }
    \label{fig:celebtsne}
\end{figure*}

==> resource/fig/tsne_cub/cub_tsne.tex <==
\begin{figure*}[t]
  \centering
%    \begin{center}
    %\framebox[4.0in]{$\;$}
    \subfigure[Feature map from first block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_cub/layer1_cub.pdf}
      \label{fig:cubsub1}
    }
    \subfigure[Feature map from second block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_cub/layer2_cub.pdf}
    %  \subcaption{A subfigure}
      \label{fig:cubsub2}
    }
        \subfigure[Feature map from fourth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_cub/layer4_cub.pdf}
    %  \subcaption{A subfigure}
      \label{fig:cubsub4}
    }    
        \subfigure[Feature map distilled in DeTT]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_cub/layer6_cub.pdf}
    %  \subcaption{A subfigure}
      \label{fig:cubsub6}
    }    
    
    \caption{
    In lower feature map, data classification is dominant to background feature (orange-green pair and red-blue pair).
    It means that it is not necessary to distill lower level feature map.
    }
    \label{fig:cubtsne}
\end{figure*}

==> resource/fig/tsne_jigsaw/jigsaw_tsne.tex <==
\begin{figure*}[t]
  \centering
%    \begin{center}
    %\framebox[4.0in]{$\;$}
    \subfigure[Feature map from third block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer3_jigsaw.pdf}
      \label{fig:jigsawsub3}
    }
    \subfigure[Feature map from fourth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer4_jigsaw.pdf}
      \label{fig:jigsawsub4}
    }
    \subfigure[Feature map from sixth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer6_jigsaw.pdf}
      \label{fig:jigsawsub6}
    }
    \subfigure[Feature map from eightth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer8_jigsaw.pdf}
      \label{fig:jigsawsub8}
    }
    \subfigure[Feature map from tenth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer10_jigsaw.pdf}
      \label{fig:jigsawsub10}
    }
    \subfigure[Feature map distilled in DeTT]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_jigsaw/layer12_jigsaw.pdf}
      \label{fig:jigsawsub12}
    } 
    
    \caption{
    In lower feature map, data classification is dominant to background feature (orange-green pair and red-blue pair).
    It means that it is not necessary to distill lower level feature map.
    }
    \label{fig:jigsawtsne}
\end{figure*}

==> resource/fig/tsne_mnli/mnli_tsne.tex <==
\begin{figure*}[t]
  \centering
%    \begin{center}
    %\framebox[4.0in]{$\;$}
    \subfigure[Feature map from fourth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_mnli/layer4_mnli.pdf}
      \label{fig:mnliwsub4}
    }
    \subfigure[Feature map from eighth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_mnli/layer8_mnli.pdf}
      \label{fig:mnliwsub8}
    }
    \subfigure[Feature map from tenth block output]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_mnli/layer10_mnli.pdf}
      \label{fig:mnliwsub10}
    }
    \subfigure[Feature map distilled in DeTT]{
      \includegraphics[width=0.47\textwidth]{resource/fig/tsne_mnli/layer12_mnli.pdf}
      \label{fig:mnlisub12}
    } 
    
    \caption{
    In lower feature map, data classification is dominant to background feature (orange-green pair and red-blue pair).
    It means that it is not necessary to distill lower level feature map.
    }
    \label{fig:mnlitsne}
\end{figure*}

==> resource/table/depth_wise/FeatureDistillAbla.tex <==
\begin{table}[t]
    \caption{Distillation performance according to distillation type.
    Vanilla KD means knowledge distillation algorithm suggested in \citep{hinton2015distilling}.
    Samples are upweighted to 50 as previously done for all tests.
    }
    \label{table:ablaFD}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{FKD} &\multirow{2}{*}{Up}& \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA}  \\
                     \cmidrule(lr{1em}){4-7}
                      &  &  & Avg Acc & WGA & Avg Acc & WGA\\
                      \midrule
                      Teacher & - & - & 91.9 & 90.8 & 92.9 & 90.6 \\
                    \midrule
                    \multirow{2}{*}{DeTT(ours)} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\cmark} & 92.1 & 88.6 & 92.9 & 89.5 \\
                     &  &  & \tiny ($\pm 0.40$) & \tiny ($\pm 0.46$) & \tiny ($\pm 0.10$) & \tiny ($\pm 1.78$) \\ 
                     \multirow{2}{*}{SimKD} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\xmark} & 89.3 & 84.5 & 93.3 & 86.9 \\
                     &  &  & \tiny ($\pm 0.10$) & \tiny ($\pm 0.78$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.86$) \\ 
                    \multirow{2}{*}{KD ($\alpha=1$)} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} & 88.5 & 86.1 &  & 87.2 \\
                     &  &  & \tiny ($\pm 0.92$) & \tiny ($\pm 0.69$) & \tiny ($\pm 0.50$) & \tiny ($\pm 1.65$) \\
                    \multirow{2}{*}{KD ($\alpha=1$)} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & 88.9 & 83.9 &  & 87.6 \\
                     &  &  & \tiny ($\pm 0.17$) & \tiny ($\pm 0.44$) & \tiny ($\pm 0.25$) & \tiny ($\pm 2.10$) \\
                    \bottomrule 
                    \end{tabular}
                    }
                \end{sc}
            \end{small}

        \end{center}
    \vskip -0.1in
\end{table}

==> resource/table/depth_wise/MainTable.tex <==
\begin{table*}[hbt!]
    \caption{
    DeTT results compared with existing robust training methods are reported in this table to check how our method can distill debiased knowledge. 
    For knowledge distillation baseline, student network is trained with vanilla knowledge distillation \cite{hinton2015distilling}. Hyperparameter $\alpha$ is ratio of KL divergence loss in ~\cref{eq:distillation}. 
    As a core baseline, JTT \cite{liu2021just} and gDRO \cite{sagawa2019distributionally} results are reported for same architecture for student network.
    Annotation column in table is about training set.
    Small validation set for early stopping has group annotation for all experiments.
}
    \label{table:main}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{\textwidth}{!}
                    {
                    \begin{tabular}{lccccccccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{Annotation} & \multirow{2}{*}{Teacher}& \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA} & \multicolumn{2}{c}{CivilComments} & \multicolumn{2}{c}{MultiNLI} \\
                     \cmidrule(lr{1em}){4-11}
                      &  &  & Average & Worst & Average & Worst & Average & Worst & Average & Worst\\
                      \midrule
                      Teacher & \cmark & \xmark & 92.4 & 90.0 & 92.0 & 89.4 & 85.0 & 78.9 & 80.3 & 78.8\\
%                    \cmidrule(lr{1em}){1-1}
                    \midrule
                     \multirow{2}{*}{group DRO} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\xmark} & 87.0 & 81.1 & 93.0 & 86.4 & 82.2 & \textbf{77.3} & 50.7 & 47.5\\
                    & &  & \tiny ($\pm 1.65$) & \tiny ($\pm 1.60$) & \tiny ($\pm 0.31$) & \tiny ($\pm 1.27$) & \tiny ($\pm 0.80$) & \tiny ($\pm 0.81$) & \tiny ($\pm 1.73$) & \tiny ($\pm 1.33$)\\
                    \midrule
                    \multirow{2}{*}{ERM} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & 75.0 & 33.8 & 95.9 & 44.1 & 91.0 & 57.5 & 50.7 & 14.1 \\
                    & &  & \tiny ($\pm 1.07$) & \tiny ($\pm 3.57$) & \tiny ($\pm 0.12$) & \tiny ($\pm 1.41$) & \tiny ($\pm 0.47$) & \tiny ($\pm 5.23$) & \tiny ($\pm 1.04$) & \tiny ($\pm 5.11$)\\
                     \multirow{2}{*}{JTT} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\xmark} & 86.7 & 80.5 & 86.4 & 77.8 & 84.0 & 60.0 & 55.1 & 25.2\\
                    & &  & \tiny ($\pm 0.50$) & \tiny ($\pm 0.53$) & \tiny ($\pm 4.65$) & \tiny ($\pm 2.48$) & \tiny ($\pm 3.21$) & \tiny ($\pm 2.06$) & \tiny ($\pm 0.89$) & \tiny ($\pm 3.44$)\\
                     \multirow{2}{*}{KD($\alpha=0.5$)} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} &  &  &  &  & 87.5 & 69.1 & 57.5 & 46.2\\
                      & &  & \tiny ($\pm $) & \tiny ($\pm $) & \tiny ($\pm 0.61$) & \tiny ($\pm 2.63$) & \tiny ($\pm 2.94$) & \tiny ($\pm 6.47$) & \tiny ($\pm 0.50$) & \tiny ($\pm 0.17$)\\
                      \multirow{2}{*}{KD($\alpha=1$)} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} & 88.9 & 83.9 &  &  & 85.0 & 74.0 & 57.3 & 51.0\\
                     & &  & \tiny ($\pm 0.17$) & \tiny ($\pm 0.44$) & \tiny ($\pm 0.25$) & \tiny ($\pm 2.10$) & \tiny ($\pm 0.50$) & \tiny ($\pm 1.04$) & \tiny ($\pm 0.31$) & \tiny ($\pm 1.39$)\\
                    \multirow{2}{*}{SimKD} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} & 89.3 & 84.5 & 93.3 & 86.9 & 87.0 & 74.0 & 70.7 & 64.1 \\
                    & &  & \tiny ($\pm 0.10$) & \tiny ($\pm 0.78$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.86$) & \tiny ($\pm 0.40$) & \tiny ($\pm 2.25$) & \tiny ($\pm 0.92$) & \tiny ($\pm 1.62$) \\
                    \midrule
                    
                    \multirow{2}{*}{DeTT(ours)} & \multirow{2}{*}{\xmark} & \multirow{2}{*}{\cmark} & 92.1 & \textbf{88.6} & 92.9 & \textbf{89.8} & 86.7 & 75.0 & 70.8 & \textbf{64.7} \\
                    & &  & \tiny ($\pm 0.40$) & \tiny ($\pm 0.46$) & \tiny ($\pm 0.10$) & \tiny ($\pm 1.78$) & \tiny ($\pm 0.56$) & \tiny ($\pm 2.56$) & \tiny ($\pm 0.81$) & \tiny ($\pm 1.55$) \\

%                    \multirow{2}{*}{KD(Pred + FKD)} & \multirow{2}{*}{No}&  &  &  &  &  &  &  &  & \\
%                    &  &  &  &  &  &  &  &  & \\
%                     LfF & No & 91.2 & 78.0 & 85.1 & 77.2 & - & - & - & -\\
%                     DFR & Yes & 94.2 & 92.9 & 91.3 & 88.3 & - & 79 & - & 73 \\
%                     SUBG & Yes & - & 89.1 & - & 85.6 & - & 71.8 & - & 68.9 \\
%                    \cmidrule(lr{1em}){1-1}
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table*}

==> resource/table/depth_wise/UpweightAbla.tex <==
\begin{table}[t]
    \caption{Feature distillation and classifier reuse results with and without sample upweighting.
    Zero upweight hyperparameter $\lambda_{up}$ (first student row) means that it distills feature using original biased dataset.
    }
    \label{table:ablaUpweight}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lcccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{$\lambda_{up}$} & \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA}  \\
                     \cmidrule(lr{1em}){3-6}
                      &  & Average & Worst & Average & Worst\\
                      \midrule
                      Teacher & - & 92.4 & 90.0 & 92.0 & 89.4 \\
                    \midrule
                    \multirow{2}{*}{SimKD} & \multirow{2}{*}{0} & 89.3 & 85.4 & 93.3 & 86.9 \\
                     &  & \tiny ($\pm 0.10$) & \tiny ($\pm 0.78$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.86$)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{5} & 90.3 & 87.5 & 93.3 & 87.4 \\
                     &  & \tiny ($\pm 0.11$) & \tiny ($\pm 0.10$) & \tiny ($\pm 0.15$) & \tiny ($\pm 0.35$)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{20} & 91.5 & 88.6 & 92.5 & 88.0 \\
                     &  & \tiny ($\pm 0.15$) & \tiny ($\pm 0.49$) & \tiny ($\pm 1.00$) & \tiny ($\pm 3.52$)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{50} & 92.1 & 88.6 & 92.9 & 89.8 \\
                     &  & \tiny ($\pm 0.40$) & \tiny ($\pm 0.46$) & \tiny ($\pm 0.10$) & \tiny ($\pm 1.78$)\\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}

==> resource/table/depth_wise/distillood.tex <==
\begin{table}[t]
    \caption{Group distribution and its group-wise accuracy of student model distilled by ImageNet dataset. 
    Num represents group distribution of original dataset (i.e. WaterBirds and CelebA, respectively)
    All notation is same with Table \ref{table:distillpatternup}.
    }
    \label{table:distillood}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lcr}
                    \toprule
                    Waterbirds & \# Samples & \multicolumn{1}{c}{$T \xrightarrow[]{\text{ImageNet}} S$} \\
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 3498 & 94.1 $\rightarrow$ 92.3 \tiny ($\pm 0.62$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 184 & 91.6 $\rightarrow$ \textbf{87.7} \tiny ($\pm 2.38$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & 56 & \textbf{90.0} $\rightarrow$ 87.8 \tiny ($\pm 0.29$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 1057 & 91.3 $\rightarrow$ 89.5 \tiny ($\pm 0.91$) \\
                    \midrule
                    CelebA &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 71629 & 92.2 $\rightarrow$ 91.0 \tiny ($\pm 1.27$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 66874 & 92.2 $\rightarrow$ 90.4 \tiny ($\pm 2.36$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 22880 & 93.7 $\rightarrow$ 91.4 \tiny ($\pm 1.04$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 1387 & \textbf{89.4} $\rightarrow$ \textbf{81.8} \tiny ($\pm 4.21$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}




==> resource/table/depth_wise/distillpattern.tex <==
\begin{table}[t]
    \caption{Group distribution and its group-wise accuracy of student model distilled without upweighting. 
    All notation is same with Table \ref{table:distillpatternup}
    }
    \label{table:distillpattern}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccr}
                    \toprule
                    Waterbirds & \# Samples & ERM & \multicolumn{1}{c}{$T \xrightarrow[]{\mathcal{X}} S$} \\
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 3498 & 98.2 & 94.1 $\rightarrow$ 93.5 \tiny ($\pm 0.45$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 184 & 58.0 & 91.6 $\rightarrow$ \textbf{85.4} \tiny ($\pm 0.78$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & \textbf{56} & \textbf{33.8} & \textbf{90.0} $\rightarrow$ 86.7 \tiny ($\pm 0.71$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 1057 & 94.4 & 91.3 $\rightarrow$ 91.5 \tiny ($\pm 0.53$) \\
                    \midrule
                    CelebA &  &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 71629 & 96.0 & 92.2 $\rightarrow$ 93.6 \tiny ($\pm 0.29$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 66874 & 99.5 & 92.2 $\rightarrow$ 93.6 \tiny ($\pm 0.40$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 22880 & 89.2 & 93.7 $\rightarrow$ 92.1 \tiny ($\pm 0.40$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 1387 & \textbf{45.6} & \textbf{89.4} $\rightarrow$ \textbf{86.9} \tiny ($\pm 0.86$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}


==> resource/table/depth_wise/distillpattern_up.tex <==
\begin{table}[t]
    \caption{Group distribution and its group-wise accuracy from our experiment. 
    In this table, sample number of each group is that of upweighted dataset.
    ERM training result with $\mathcal{X}_{\mathrm{up}}$ is identical with JTT.
    Label is represented as (class label, feature annotation).
    For Waterbirds, class label is type of bird.
    Feature annotation \texttt{water} and \texttt{land} is \texttt{water-background} and \texttt{land-background}. 
    }
    \label{table:distillpatternup}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccr}
                    \toprule
                    Waterbirds & \# Samples & ERM & \multicolumn{1}{c}{$T \xrightarrow[]{\mathcal{X}_{\mathrm{up}}} S$} \\ 
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 4298 & 92.7 & 94.1 $\rightarrow$ 94.7 \tiny ($\pm 0.80$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 6084 & \textbf{80.5} & 91.6 $\rightarrow$ 91.3 \tiny ($\pm 0.35$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & 4656 & 83.2 & \textbf{90.0} $\rightarrow$ \textbf{88.6} \tiny ($\pm 0.46$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 12257 & 90.5 & 91.3 $\rightarrow$ 90.1 \tiny ($\pm 1.39$) \\
                    \midrule
                    CelebA &  &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 200329 & 84.3 & 92.2 $\rightarrow$ 93.0 \tiny ($\pm 0.15$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 673024 & 89.7 & 92.2 $\rightarrow$ 92.9 \tiny ($\pm 0.15$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 466980 & 84.5 & 93.7 $\rightarrow$ 93.0 \tiny ($\pm 0.31$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 63837 & \textbf{80.4} & \textbf{89.4} $\rightarrow$ \textbf{89.8} \tiny ($\pm 1.78$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}


==> resource/table/rn18/FeatureDistillAbla.tex <==
\begin{table}[t]
    \caption{Distillation performance according to distillation type.
    Vanilla KD means knowledge distillation algorithm suggested in \citep{hinton2015distilling}.
    Samples are upweighted to 50 as previously done for all tests.
    }
    \label{table:ablaFD}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{FKD} &\multirow{2}{*}{Up}& \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA}  \\
                      &  &  & Avg Acc & WGA & Avg Acc & WGA\\
                      \midrule
                      Teacher & - & - & 91.9 & 90.8 & 92.9 & 90.6 \\
                    \cmidrule(lr{1em}){1-1}
                    \multirow{2}{*}{DeTT(ours)} & \multirow{2}{*}{\checkmark} & \multirow{2}{*}{\checkmark} & 92.3 & 88.4 & 93.0 & 88.3 \\
                     &  &  & \tiny ($\pm 0.32$) & \tiny ($\pm 0.78$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.55$) \\ 
                     \multirow{2}{*}{SimKD} & \multirow{2}{*}{\checkmark} &  & 89.7 & 85.4 & 93.3 & 87.4 \\
                     &  &  & \tiny ($\pm 0.36$) & \tiny ($\pm 0.42$) & \tiny ($\pm 0.11$) & \tiny ($\pm 0.35$) \\
                    \multirow{2}{*}{Vanilla KD} &  & \multirow{2}{*}{\checkmark} & 86.9 & 84.3 & 93.2 & 87.2 \\
                     &  &  & \tiny ($\pm 2.49$) & \tiny ($\pm 1.82$) & \tiny ($\pm 0.50$) & \tiny ($\pm 1.65$) \\
                    \multirow{2}{*}{Vanilla KD} &  &  & 88.6 & 83.5 & 93.3 & 87.6 \\
                     &  &  & \tiny ($\pm 0.74$) & \tiny ($\pm 0.97$) & \tiny ($\pm 0.25$) & \tiny ($\pm 2.10$) \\
                    \bottomrule 
                    \end{tabular}
                    }
                \end{sc}
            \end{small}

        \end{center}
    \vskip -0.1in
\end{table}

==> resource/table/rn18/MainTable.tex <==
\begin{table*}[hbt!]
    \caption{
    DeTT results compared with existing robust training methods are reported in this table to check how our method can distill debiased knowledge. 
    For knowledge distillation baseline, student network is trained with vanilla knowledge distillation \cite{hinton2015distilling}. Hyperparameter $\alpha$ is ratio of KLDiv loss in total loss. 
    As a core baseline, JTT \cite{liu2021just} and gDRO \cite{sagawa2019distributionally} results are reported for same architecture for student network.
    Annotation column in table is about training set.
    Small validation set for early stopping has group annotation for all experiments.
}
    \label{table:main}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{\textwidth}{!}
                    {
                    \begin{tabular}{lccccccccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{Annotation} & \multirow{2}{*}{Teacher}& \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA} & \multicolumn{2}{c}{CivilComments} & \multicolumn{2}{c}{MultiNLI} \\
                      &  &  & Average & Worst & Average & Worst & Average & Worst & Average & Worst\\
                      \midrule
                      Teacher & \cmark & \xmark & 92.4 & 90.0 & 92.0 & 89.4 & 85.0 & 78.9 & 80.3 & 78.8\\
%                    \cmidrule(lr{1em}){1-1}
                    \midrule
                     \multirow{2}{*}{group DRO} & \multirow{2}{*}{\checkmark} &  & 87.0 & 80.0 & 92.9 & 87.6 & 82.2 & \textbf{77.3} & 50.7 & 47.5\\
                    & &  & \tiny ($\pm 0.91$) & \tiny ($\pm 1.65$) & \tiny ($\pm 0.35$) & \tiny ($\pm 1.15$) & \tiny ($\pm 0.80$) & \tiny ($\pm 0.81$) & \tiny ($\pm 1.73$) & \tiny ($\pm 1.33$)\\
                    \midrule
                    \multirow{2}{*}{ERM} & \multirow{2}{*}{}& \multirow{2}{*}{} & 71.5 & 18.6 & 96.0 & 45.6 & 91.0 & 57.5 & 50.7 & 14.1 \\
                    & &  & \tiny ($\pm 0.91$) & \tiny ($\pm 0.77$) & \tiny ($\pm 0.06$) & \tiny ($\pm 2.12$) & \tiny ($\pm 0.47)$ & \tiny ($\pm 5.23$) & \tiny ($\pm 1.04$) & \tiny ($\pm 5.11$)\\
                     \multirow{2}{*}{JTT} & \multirow{2}{*}{}& \multirow{2}{*}{} & 86.8 & 81.8 & 89.3 & 78.3 & 84.0 & 60.0 & 55.1 & 25.2\\
                    & &  & \tiny ($\pm 0.50$) & \tiny ($\pm 0.96$) & \tiny ($\pm 2.75$) & \tiny ($\pm 1.48$) & \tiny ($\pm 3.21$) & \tiny ($\pm 2.06$) & \tiny ($\pm 0.89$) & \tiny ($\pm 3.44$)\\
                     \multirow{2}{*}{KD($\alpha=0.5$)} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & 57.2 & 14.6 & 94.4 & 75.2 & 87.5 & 69.1 &  & \\
                      & &  & \tiny ($\pm 2.39$) & \tiny ($\pm 0.91$) & \tiny ($\pm 0.61$) & \tiny ($\pm 2.63$) & \tiny ($\pm 2.94$) & \tiny ($\pm 6.47$) &  & \\
                      \multirow{2}{*}{KD($\alpha=1$)} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & 88.6 & 83.5 & 93.3 & 87.6 & 85.0 & 74.0 & 57.3 & 51.0\\
                     & &  & \tiny ($\pm 0.74$) & \tiny ($\pm 0.97$) & \tiny ($\pm 0.25$) & \tiny ($\pm 2.10$) & \tiny ($\pm 0.50$) & \tiny ($\pm 1.04$) & \tiny ($\pm 0.31$) & \tiny ($\pm 1.39$)\\
                    \multirow{2}{*}{SimKD} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & 89.7 & 85.4 & 93.3 & 87.4 & 87.0 & 74.0 & 70.7 & 64.1 \\
                    & &  & \tiny ($\pm 0.36$) & \tiny ($\pm 0.42$) & \tiny ($\pm 0.11$) & \tiny ($\pm 0.35$) & \tiny ($\pm 0.40$) & \tiny ($\pm 2.25$) & \tiny ($\pm 0.92$) & \tiny ($\pm 1.62$) \\
                    \midrule
                    
                    \multirow{2}{*}{DeTT(ours)} & \multirow{2}{*}{} & \multirow{2}{*}{\checkmark} & 91.3 & \textbf{89.1} & 93.0 & \textbf{88.3} & 86.7 & 75.0 & 70.8 & \textbf{64.7} \\
                    & &  & \tiny ($\pm 0.06$) & \tiny ($\pm 0.44$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.55$) & \tiny ($\pm 0.56$) & \tiny ($\pm 2.56$) & \tiny ($\pm 0.81$) & \tiny ($\pm 1.55$) \\

%                    \multirow{2}{*}{KD(Pred + FKD)} & \multirow{2}{*}{No}&  &  &  &  &  &  &  &  & \\
%                    &  &  &  &  &  &  &  &  & \\
%                     LfF & No & 91.2 & 78.0 & 85.1 & 77.2 & - & - & - & -\\
%                     DFR & Yes & 94.2 & 92.9 & 91.3 & 88.3 & - & 79 & - & 73 \\
%                     SUBG & Yes & - & 89.1 & - & 85.6 & - & 71.8 & - & 68.9 \\
%                    \cmidrule(lr{1em}){1-1}
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table*}

==> resource/table/rn18/UpweightAbla.tex <==
\begin{table}[hbt!]
    \caption{Feature distillation and classifier reuse results with and without sample upweighting.
    Zero upweight hyperparameter $\lambda_{up}$ (first student row) means that it distills feature using original biased dataset.
    }
    \label{table:ablaUpweight}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lcccccr}
                    \toprule
                     \multirow{2}{*}{Method} & \multirow{2}{*}{$\lambda_{up}$} & \multicolumn{2}{c}{Waterbirds} & \multicolumn{2}{c}{CelebA}  \\
                      &  & Average & Worst & Average & Worst\\
                      \midrule
                      Teacher & - & 92.4 & 90.0 & 92.0 & 89.4 \\
                    \cmidrule(lr{1em}){1-1}
                    \multirow{2}{*}{SimKD} & \multirow{2}{*}{0} & 89.7 & 85.4 & 93.3 & 87.4 \\
                     &  & \tiny ($\pm 0.36$) & \tiny ($\pm 0.42$) & \tiny ($\pm 0.11$) & \tiny ($\pm 0.35$)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{5} & 90.6 & 87.7 &  &  \\
                     &  & \tiny ($\pm 0.20$) & \tiny ($\pm 0.50$) & \tiny ($\pm $) & \tiny ($\pm $)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{20} & 91.3 & 89.1 &  &  \\
                     &  & \tiny ($\pm 0.06$) & \tiny ($\pm 0.44$) & \tiny ($\pm $) & \tiny ($\pm $)\\
                    \multirow{2}{*}{DeTT} & \multirow{2}{*}{50} & 92.1 & 88.4 & 93.0 & 88.3 \\
                     &  & \tiny ($\pm 0.32$) & \tiny ($\pm 0.78$) & \tiny ($\pm 0.26$) & \tiny ($\pm 0.55$)\\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}

==> resource/table/rn18/distillood.tex <==
\begin{table}[hbt!]
    \caption{Group distribution and its group-wise accuracy of student model distilled by ImageNet dataset. 
    Num represents group distribution of original dataset (i.e. WaterBirds and CelebA, respectively)
    All notation is same with Table \ref{table:distillpatternup}.
    }
    \label{table:distillood}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lcr}
                    \toprule
                    Waterbirds & \# Samples & \multicolumn{1}{c}{$T \xrightarrow[]{\text{ImageNet}} S$} \\
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 3498 & 94.1 $\rightarrow$ 92.6 \tiny  ($\pm 0.40$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 184 & 91.6 $\rightarrow$ 88.6 \tiny($\pm 0.76$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & 56 & \textbf{90.0} $\rightarrow$ \textbf{88.2} \tiny($\pm 0.31$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 1057 & 91.3 $\rightarrow$ 90.2 \tiny($\pm 0.17$) \\
                    \midrule
                    CelebA &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 71629 & 92.2 $\rightarrow$ 93.3 \tiny ($\pm 2.34$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 66874 & 92.2 $\rightarrow$ 92.4 \tiny ($\pm 2.54$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 22880 & 93.7 $\rightarrow$ 89.0 \tiny ($\pm 5.84$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 1387 & \textbf{89.4} $\rightarrow$ \textbf{76.3} \tiny ($\pm 9.07$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}




==> resource/table/rn18/distillpattern.tex <==
\begin{table}[hbt!]
    \caption{Group distribution and its group-wise accuracy of student model distilled without upweighting. 
    All notation is same with Table \ref{table:distillpatternup}
    }
    \label{table:distillpattern}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccr}
                    \toprule
                    Waterbirds & \# Samples & ERM & \multicolumn{1}{c}{$T \xrightarrow[]{\mathcal{X}} S$} \\
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 3498 & 99.1 & 94.1 $\rightarrow$ 93.9 \tiny ($\pm 0.29$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 184 & 53.3 & 91.6 $\rightarrow$ \textbf{85.4} \tiny ($\pm 0.42$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & \textbf{56} & \textbf{18.6} & \textbf{90.0} $\rightarrow$ 89.0 \tiny ($\pm 0.63$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 1057 & 91.7 & 91.3 $\rightarrow$ 91.7 \tiny ($\pm 0.66$) \\
                    \midrule
                    CelebA &  &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 71629 & 96.0 & 92.2 $\rightarrow$ 93.4 \tiny ($\pm 0.11$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 66874 & 99.5 & 92.2 $\rightarrow$ 93.3 \tiny ($\pm 0.23$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 22880 & 89.2 & 93.7 $\rightarrow$ 92.7 \tiny ($\pm 0.28$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 1387 & \textbf{45.6} & \textbf{89.4} $\rightarrow$  \textbf{87.4} \tiny ($\pm 0.35$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}


==> resource/table/rn18/distillpattern_up.tex <==
\begin{table}[hbt!]
    \caption{Group distribution and its group-wise accuracy from our experiment. 
    In this table, sample number of each group is that of upweighted dataset.
    ERM training result with $\mathcal{X}_{\mathrm{up}}$ is identical with JTT.
    Label is represented as (class label, feature annotation).
    For Waterbirds, class label is type of bird.
    Feature annotation \texttt{water} and \texttt{land} is \texttt{water-background} and \texttt{land-background}. 
    }
    \label{table:distillpatternup}
    \vskip 0.15in
        \begin{center}
            \begin{small}
                \begin{sc}
                    \resizebox{0.47\textwidth}{!}
                    {
                    \begin{tabular}{lccr}
                    \toprule
                    Waterbirds & Num & ERM & \multicolumn{1}{c}{$T \xrightarrow[]{\mathcal{X}_{\mathrm{up}}} S$} \\ 
                    \midrule
                    ($\mathtt{waterbirds}$,$\mathtt{water}$) & 4298 & 92.6 & 94.1 $\rightarrow$ 94.9 \tiny ($\pm 0.44$) \\
                    ($\mathtt{waterbirds}$,$\mathtt{land}$) & 6084 & \textbf{81.8} & 91.6 $\rightarrow$ 91.7 \tiny ($\pm 0.66$) \\
                    ($\mathtt{landbirds}$,$\mathtt{water}$) & 4656 & 82.5 & \textbf{90.0} $\rightarrow$ \textbf{88.4} \tiny ($\pm 0.78$) \\
                    ($\mathtt{landbirds}$,$\mathtt{land}$) & 12257 & 88.3 & 91.3 $\rightarrow$ 89.5 \tiny ($\pm 0.53$) \\
                    \midrule
                    CelebA &  &  &   \\
                    \midrule
                    ($\mathtt{nonblond}$,$\mathtt{female}$) & 200329 & 87.2 & 92.2 $\rightarrow$ 93.2 \tiny ($\pm 0.32$) \\
                    ($\mathtt{nonblond}$,$\mathtt{male}$) & 673024 & 93.6 & 92.2 $\rightarrow$ 92.9 \tiny ($\pm 0.42$) \\
                    ($\mathtt{blond}$,$\mathtt{female}$) & 466980 & 84.9 & 93.7 $\rightarrow$ 92.9 \tiny ($\pm 0.36$) \\
                    ($\mathtt{blond}$,$\mathtt{male}$) & 63837 & \textbf{78.3} & \textbf{89.4} $\rightarrow$ \textbf{88.3} \tiny ($\pm 0.55$) \\
                    \bottomrule
                    \end{tabular}
                    }
                \end{sc}
            \end{small}
        \end{center}
    \vskip -0.1in
\end{table}

